Evaluating Code Summarization Techniques: A New Metric and an Empirical Characterization

Several code summarization techniques have been proposed in the literature to automatically document a code snippet or a function. Ideally, software developers should be involved in assessing the quality of the generated summaries. However, in most cases, researchers rely on automatic evaluation metrics such as BLEU, ROUGE, and METEOR. These metrics are all based on the same assumption: The higher the textual similarity between the generated summary and a reference summary written by developers, the higher its quality. However, there are two reasons for which this assumption falls short: (i) reference summaries, e.g., code comments collected by mining software repositories, may be of low quality or even outdated; (ii) generated summaries, while using a different wording than a reference one, could be semantically equivalent to it, thus still being suitable to document the code snippet. In this paper, we perform a thorough empirical investigation on the complementarity of different types of metrics in capturing the quality of a generated summary. Also, we propose to address the limitations of existing metrics by considering a new dimension, capturing the extent to which the generated summary aligns with the semantics of the documented code snippet, independently from the reference summary. To this end, we present a new metric based on contrastive learning to capture said aspect. We empirically show that the inclusion of this novel dimension enables a more effective representation of developers' evaluations regarding the quality of automatically generated summaries.

==> tables/cosine_similarity.tex <==
% !TEX root = ../main.tex

% Design tables. 

\begin{table}[ht]
	\centering
	\caption{Reported results in terms of cosine similarity for each tested configuration.}
	\scriptsize
	\label{tab:cosine}
	\begin{tabular}{llrr}
	\toprule
	{\bf Data} & {\bf Dataset} & {\bf Best-Performing } & {\bf Cosine }\\
	{\bf  Augmentation} & {\bf  Size} & {\bf  Checkpoint} & {\bf  Similarity}\\\midrule
	 DA$_{null}$  & & 103,080 & 0.828 \\
	 DA0 & & 185,000 & 0.819\\
	 DA1 & & 141,205 & 0.817 \\
	 DA0 + DA1 & & 255,000& 0.804 \\
\bottomrule
\end{tabular} 
\end{table}
